Dynamic Localisation of Spatial-Temporal Graph Neural Network

Spatial-temporal data, fundamental to many intelligent applications, reveals dependencies indicating causal links between present measurements at specific locations and historical data at the same or other locations. Within this context, adaptive spatial-temporal graph neural networks (ASTGNNs) have emerged as valuable tools for modelling these dependencies, especially through a data-driven approach rather than pre-defined spatial graphs. While this approach offers higher accuracy, it presents increased computational demands. Addressing this challenge, this paper delves into the concept of localisation within ASTGNNs, introducing an innovative perspective that spatial dependencies should be dynamically evolving over time. We introduce \textit{DynAGS}, a localised ASTGNN framework aimed at maximising efficiency and accuracy in distributed deployment. This framework integrates dynamic localisation, time-evolving spatial graphs, and personalised localisation, all orchestrated around the Dynamic Graph Generator, a light-weighted central module leveraging cross attention. The central module can integrate historical information in a node-independent manner to enhance the feature representation of nodes at the current moment. This improved feature representation is then used to generate a dynamic sparse graph without the need for costly data exchanges, and it supports personalised localisation. Performance assessments across two core ASTGNN architectures and nine real-world datasets from various applications reveal that \textit{DynAGS} outshines current benchmarks, underscoring that the dynamic modelling of spatial dependencies can drastically improve model expressibility, flexibility, and system efficiency, especially in distributed settings.

==> body/method.tex <==
\section{Method}
% \subsection{\sysname Overview}
% \label{sec:method:overview}
%\figref{} depicts the overview of \sysname. It mainly consists of two modules.
% Our \sysname mainly consists of two modules.
% \begin{itemize}
%     \item \textit{Node-Specific Transformer}:
%     %Let $\mathcal{X}_{i}^{{T}_{r}}$ be the rest history data of $\mathcal{X}_{i}^{{T}_{h}}$ from node $i$. 
%     %For the $i$-th node at timestep $t$, The meta layers take $\mathcal{X}_{i}^{{T}_{r}}$ and $X_{i,t} \in \mathcal{X}_{i}^{{T}_{h}}$ as input and output a representation.  The representation is then used to \textit{i)} determine whether node $i$ needs to aggregate information from other nodes and textit{i)} inject into the main layers to generate the adaptive adjacency matrix at timestep $t$. We employ transformer for the meta layers (see \secref{}).

%     At current timestep $t$, the node-specific Transformer then takes the current input of ASTGNN (decoder inputs) and its corresponding rest history data (encoder inputs) as inputs, and outputs a representation.
    
%     For the $i$-th node, the weights of Transformer are generated by hypernetworks which takes the $i$-th node embedding $\mathbf{e}_{i}$ as input, so it is called Node-Specific Transformer.
%     At current timestep $t$, the node-specific Transformer then takes the current input of ASTGNN (decoder inputs) and its corresponding rest history data (encoder inputs) as inputs, and outputs a representation. The representation is then used to \textit{i)} determine whether node $i$ needs to aggregate information from other nodes and \textit{ii)} injects into ASTGNNs to generate a dynamic adaptive adjacency matrix at timestep $t$. (see \secref{sec:nstf}).
%     \item \textit{ASTGNNs}: In our experiments, we chose AGCRN and STG-NCDE for forecasting task, as well as DVGCRN for anomaly detection task. ASTGNNs adapt their localisation according to the output representations of the node-specific Transformer. (see \secref{sec:mainlayer})
% \end{itemize}
% The interaction between the node-Specific Transformer and ASTGNNs is illustrated in \figref{fig:overview}.
% \begin{figure*}[t]
%     \centering
%     \includegraphics[width=0.9\linewidth]{figures/WWW106_V2.pdf}
%     \caption{}
%     \label{fig:overview}
% \end{figure*}
To enable dynamic localisation, it is necessary to generate the time-evolving mask matrix $\mathbf{M}_{t}$ and adaptive adjacency matrix $\mathbf{A}_{t}^{adp}$ as mentioned in \secref{subsec:gcn}. To achieve this, we have designed a framework, \sysname, built around a core module known as the \textit{Dynamic Graph Generator (DGG)}. 

%This module consists of a group of node-specific transformers, each assigned to an individual node. Each transformer processes locally available historical data to determine the incoming weights and connections of its associated node.
%In addition, echoing the embedding concept from AGCRN~\cite{bib:NIPS20:Bai}, the parameters of the node-specific transformers are not learned directly, but rather generated by a set of trainable hypernetworks. These hypernetworks, shared among all nodes, takes the node-specific embedding $\mathbf{e}_{i}$ (as introduced in \secref{subsec:gcn}) as input and generate the parameters for the $i$-th transformer, associated with the $i$-th node. Consequently, knowledge is softly shared among all node-specific transformers, similar to the node-specific weights in AGCRN.

% An overview of the \sysname framework is provided in \figref{fig:overview}.

% For the $i$-th node and at the time $t$, each transformer takes the current data $\Mathbf{X}_{i,t} \in $

% \begin{itemize}
%     \item \textit{Dynamic Graph Generator (DGG)}: 
%     In order to generate the time-evolving mask matrix $\mathbf{M}_{t}$ and adjacency matrix $\mathbf{A}_{t}^{adp}$ mentioned in \secref{subsec:gcn}, we assign node-specific transformers to each node. 
%     For the $i$-th node and at the time $t$, each transformer takes the current data $\Mathbf{X}_{i,t} \in $
    
%     This is a transformer whose parameters are generated by hypernetworks, which take the node-specific embedding $\mathbf{e}_{i}$ as input.
%     Therefore, 
%     This module generates the weights of a Transformer by using hypernetworks that take the embedding $\mathbf{e}_{i}$ of the $i$-th node as input. Hence, it is termed as the Node-Specific Transformer. At the current timestep $t$, this Transformer accepts both the current input of ASTGNN (decoder inputs) and its corresponding rest history data (encoder inputs). This process results in a representation that is then used to \textit{i)} ascertain whether node $i$ requires aggregation of information from other nodes and \textit{ii)} inject into the ASTGNNs to generate a dynamic adaptive adjacency matrix at timestep $t$. More details can be found in \secref{sec:nstf}.
%     \item \textit{ASTGNNs}: 
%     For our experiments, we selected AGCRN and STG-NCDE for the forecasting task, and DVGCRN for the anomaly detection task. ASTGNNs adjust their localization according to the output representations of the Node-Specific Transformer. Further information is provided in \secref{sec:mainlayer}.
% \end{itemize}
% The interaction between the Node-Specific Transformer and ASTGNNs is illustrated in 

%For the $i$-th node, the $T_h$ historical observations at timestep $t$ are denoted as $\mathcal{X}_{i,t}^{T_{h}}=\{\mathbf{x}_{i,t-T_{h}+1}, \ldots, \mathbf{x}_{i,t}\} \in \mathbb{R}^{T_{h}\times C}$.
%Let $\mathcal{X}_{i}^{{T}_{r}} = \{\mathbf{x}_{i,t-T_{h}-T{s}+1}, \ldots, \mathbf{x}_{i,t-T_{h}}\}$\\$\in \mathbb{R}^{T_{r}\times C}$ be the rest history data of $\mathcal{X}_{i,t}^{T_{h}}$, given observation $\mathbf{x}_{i,t}$ at current timestep $t$.
%$\mathcal{X}_{i}^{{T}_{r}}$ and $\mathbf{x}_{i,t}$ are fed into the meta layers to generate a representation $h_{t}$. $h_{t}$ then generates a dynamic node embedding $\mathbf{\overline{e}_i}$ and the $i$-th column mask vector of $\mathbf{M}_{t}$, which is denoted as $\mathbf{m}_{:,i} \in \mathbb{R}^{1 \times N}$. Finally, main layers utilize all node embeddings and mask vectors to achieve adaptive localisation. 
\subsection{Dynamic Graph Generator (DGG)}
\label{sec:nstf}
As outlined in \secref{subsec:notation}, in most spatial-temporal tasks, the look-back period $T_h$ is typically much shorter than the entire time interval covered by the available data. For the $i$-th node at a chosen task time $\tau$, we define the \textit{residual historical data}:

\begin{equation}
    \mathcal{X}_{i,\tau}^{res} = \{\mathbf{X}_{i,1}, \ldots, \mathbf{X}_{i,\tau-T_h}\} \in \mathbb{R}^{T_r\times C}
\end{equation}
During inference, for the $i$-th node at timestep $t \in \{\tau-T_h+1, \cdots, \tau\}$, each transformer accepts the node-specific residual historical data $\mathcal{X}_{i,\tau}^{res}$ as the encoder input, and the observation at the moment $\mathbf{X}_{i,t} \in \mathbb{R}^{C}$ as the decoder input. The transformer then output an vector $\mathbf{h}_{i,t} \in \mathbb{R}^{ D}$, which is subsequently utilised to determine the incoming weights and connections of the corresponding node, as detailed in \secref{sec:mainlayer}. Note that in practice, we put an upper-limit on the length $T_r$ of $\mathcal{X}_{i,\tau}^{res}$ based on datasets to ensure that the computational cost is acceptable.
This may change the $\mathcal{X}_{i,\tau}^{res}$ to $\{\mathbf{X}_{i,\tau-T_h-T_r+1}, \ldots, \mathbf{X}_{i,\tau-T_h}\}$

\subsubsection{Down-sampling and Patching} 

The first challenge lies in efficiently representing the residual historical data, given that the length of this data, $T_r$, is extremely large. Several studies on time-series processing propose reducing the input length via down-sampling or patching. In this case, we employ a combination of both methods to significantly decrease the length of the encoder input. For the $i$-th node, given the residual historical data $\mathcal{X}_{i,\tau}^{res} \in \mathbb{R}^{T_r\times C}$, we first apply 1D average pooling with a kernel $k$ and stride $k$ over $\mathcal{X}_{i,\tau}^{res}$ on the time dimension to down-sample it into $\frac{1}{k}$ of its original slice:

\begin{equation}\label{eq:avgpool}
{\overline{\mathcal{X}}_{i,\tau}^{\frac{{T}_{r}}{k}}=\operatorname{AvgPool1D}\left(\mathcal{X}_{i,t}^{res}\right)} \in \mathbb{R}^{{\frac{T_r}{k}} \times C}
\end{equation}
% where $\overline{\mathcal{X}}_{i}^{\frac{{T}_{r}}{k}} $.
Next, we divide $\overline{\mathcal{X}}_{i,\tau}^{\frac{{T}_{r}}{k}}$ into $T_{p}$ non-overlapping patches of length $T_s$ to obtain a sequence of the  residual historical patches $\mathbf{X}_{i,\tau}^{p} \in \mathbb{R}^{ {T_{s} C}\times T_{p}} $.
%$\frac{{T}_{r}}{k}=T_{p}\cdot T_{s}$. The $n$-th patch is denoted as $\Hat{\mathbf{X}}_{i,n} \in \mathbb{R}^{T_{s} C}$. 
With the use of down-sampling and patching, the number of tokens can be reduced from $T_{r}$ to $\frac{T_{r}}{kT_{p}}$. 

Down-sampling and patching are applied for several reasons: 
\begin{itemize}
    \item To manage long residual historical data within time and memory constraints, down-sampling and patching are essential.
    \item Down-sampling effectively retains key periodic and seasonal information from spatial-temporal data, which often includes redundant temporal details \cite{10077946}.
    \item From a temporal perspective, spatial-temporal mining seeks to understand the correlation between data at each time step.
     Patching captures comprehensive semantic information that is not available at the point-level by aggregating time steps into subseries-level patches \cite{DBLP:conf/iclr/NieNSK23}.
\end{itemize}

%\begin{itemize}
 %   \item Given the constraints on time complexity and memory, down-sampling and patching designs enable the model to handle extremely long residual historical data.
  %  \item Spatial-temporal data often contains a significant amount of redundant temporal information. Down-sampling preserves most of the periodic and seasonal information in the residual historical data at a larger granularity \cite{10077946}.
   % \item From a temporal perspective, spatial-temporal mining seeks to understand the correlation between data at each time step. %However, a single time step does not have semantic meaning like a word in a sentence, thus extracting local semantic information is crucial in analyzing their connections. 
    %Patching enhances locality and captures comprehensive semantic information that is not available at the point-level by aggregating time steps into subseries-level patches. Please see \cite{DBLP:conf/iclr/NieNSK23} for more details.
%\end{itemize}

% The first challenge is how to efficiently represent the residual historical data since the length of residual historical data $T_r$ is extremely large. Many works on time-series processing suggest to reduce the input length by down-sampling or patching. Here we combine both down-sampling and patching to greatly reduce the length of the encoder input. For the $i$-th node, given the residual historical data $\mathcal{X}_{i}^{{T}_{r}} \in \mathbb{R}^{T_r\times C}$.
% We first apply 1D average pooling with kernel $k$ and stride $k$ over $\mathcal{X}_{i}^{{T}_{r}}$ on time dimension to down sample into its $\frac{1}{k}$ slice:
%     \begin{equation}\label{eq:avgpool}
% \medop{\overline{\mathcal{X}}_{i}^{\frac{{T}_{r}}{k}}=\operatorname{AvgPool1D}\left(\mathcal{X}_{i}^{{T}_{r}}\right)}
%     \end{equation}
% where $\overline{\mathcal{X}}_{i}^{\frac{{T}_{r}}{k}} \in \mathbb{R}^{{\frac{T_r}{k}} \times C}$.
% We then divide $\overline{\mathcal{X}}_{i}^{\frac{{T}_{r}}{k}}$ into $T_{p}$ non-overlapping patches of length $T_s$ to get the residual historical patches, \ie $\frac{{T}_{r}}{k}=T_{p}*T_{s}$. The $n$-th patch is denoted as $\Hat{\mathbf{x}}_{i,n} \in \mathbb{R}^{T_{s}C}$. With the use of down-sample and patching, the number of tokens can reduce from $T_{r}$ to $\frac{T_{r}}{kT_{p}}$. 
% Down-sampling and patching are applied for the following reasons.
% \begin{itemize}
%     \item Constrained on the time complexity and memory, down-sampling and patching designs can allow the model to very long residual historical data.
%     \item As a special type of time series, spatial-temporal data often carries heavily temporal redundant information, down-sampling preserves the most of the periodic and seasonal information in the residual historical data at a bigger granularity.
%     \item From temporal viewpoint, spatial-temporal mining aims to understand the correlation between data in each timestep. However, a single time step does not have semantic meaning like a word in a sentence, thus extracting local semantic information is essential in analyzing their connections. Pacthing enhances the locality and capture comprehensive semantic information that is not available in point-level by aggregating time steps into subseries-level patches.
    
% \end{itemize}

\subsubsection{Cross Attention}
%We utilise transformers to process the residual historical patches and standard historical observations. These patches and observations are initially processed by two trainable linear layers, aided by a learnable additive position encoding respectively. During inference, for the $i$-th node at timestep $t \in \{\tau-T_h+1, \cdots, \tau\}$:
%\begin{equation}
%\begin{aligned}
%\mathbf{u}_{i,n}&=\Hat{\mathbf{X}}_{i,n}\mathbf{W}^{u}_{i}+\mathbf{b}^{u}_{i}+\mathbf{e}_{pos}(n)\\
%\mathbf{v}_{i,t}&={\mathbf{X}}_{i,t}\mathbf{W}^{v}_{i}+\mathbf{b}^{v}_{i}+\mathbf{e}_{pos}(t)
%\end{aligned}
%\label{eq:fc}
%\end{equation}
%Here, $\mathbf{u}_{i,n} \in \mathbb{R}^D$ is calculated from the $n$-th residual historical patch $\Hat{\mathbf{X}}_{i,n}$, and $\mathbf{v}_{i,t} \in \mathbb{R}^D$ from the observation $\mathbf{X}_{i,t}$. $\mathbf{W}^{u}_{i} \in \mathbb{R}^{(T_{s}C)\times D}$, $\mathbf{b}^{u}_{i} \in \mathbb{R}^{D}$, $\mathbf{W}^{v}_{i} \in \mathbb{R}^{C\times D}$ and  $\mathbf{b}^{v}_{i} \in \mathbb{R}^{D}$ are learnable parameters. $\mathbf{e}_{pos}(n) \in \mathbb{R}^D$ and $\mathbf{e}_{pos}(t) \in \mathbb{R}^D$ represent the position vector for the $n$-th residual historical patch and timestep $t$, respectively. The output from the $n$ patches forms a sequences $\mathbf{U}_{i,\tau} = \{\mathbf{u}_{i,1}, \ldots \mathbf{u}_{i,T_p}\}$. This sequence is subsequently fed into the node-specific transformer, together with $\mathbf{v}_{i,t}$:

%\begin{equation}
%\begin{aligned}
%\mathbf{u}_{i,n}&=\Hat{\mathbf{X}}_{i,n}\mathbf{W}^{u}_{i}+\mathbf{b}^{u}_{i}+\mathbf{e}_{pos}(n)\\
%\mathbf{v}_{i,t}&={\mathbf{X}}_{i,t}\mathbf{W}^{v}_{i}+\mathbf{b}^{v}_{i}+\mathbf{e}_{pos}(t)
%\end{aligned}
%\label{eq:fc}
%\end{equation}
%\begin{equation}
%\mathbf{h}_{i,t} = \operatorname{Cross-Attention}(\mathbf{v}_{i,t},\mathbf{U}_{i,\tau}, \mathbf{U}_{i,\tau}) 
%\end{equation}
We utilise a cross-attention to process the residual historical patches and standard historical observations. These patches and observations are initially processed by two trainable linear layers, respectively. During inference, for the $i$-th node at timestep $t \in \{\tau-T_h+1, \cdots, \tau\}$:
\begin{equation}
    \mathbf{Q} =\mathbf{K}=(\mathbf{X}_{i,\tau}^{p}+\mathbf{e}_{pos})\mathbf{W}^{p}_{i}, \mathbf{V}= {\mathbf{X}}_{i,t}\mathbf{W}^{v}_{i}
\end{equation}
Then, we apply cross-attention operations in the temporal dimension to model the interaction between:
\begin{equation}
    \mathbf{h}_{i,t} =\operatorname{Softmax}({\frac{\mathbf{Q}\mathbf{K}^{^\top}}{\sqrt{d^{\prime}}}})\mathbf{V} \\
\end{equation}
In the end, the cross-attention outputs $\mathbf{h}_{i,t}$ from the $N$ nodes are stacked together to from a matrix $\mathbf{H}_{:,t} = \mathbf{h}_{1,t}, \cdots, \mathbf{h}_{N,t}\} \in \mathbb{R}^{N \times D}$. This matrix $\mathbf{H}_{:,t}$ is used later to generate the time-evolving $\mathbf{M}_{t}$ and $\mathbf{A}_{t}^{adp}$, which is explained in details in \secref{sec:mainlayer}.

In summary, our approach elevates feature initialization-based methods by fusing the current feature $\mathbf{H}{:,t}$ with insights from residual historical patches, culminating in the adaptive, time-evolving feature $\mathbf{A}{t}^{adp}$. Our methodology distinguishes itself from conventional approaches: $\mathbf{X}{i,t}$ functions as the query, whereas the sequence of residual historical patches $\mathbf{X}{i,\tau}^{p}$ constitutes both key and value. This configuration empowers our Dynamic Graph Generator (DGG) with an attention mechanism that selectively hones in on the most relevant segments of historical data, including the nuances introduced by patching.  This setup enables the attention mechanism in our DGG to selectively focus on historical data segments most pertinent to the present input. The final fused feature representation $\mathbf{H}_{:,t}$ is a rich amalgamation of current and historical data features, enhanced by patching, which is vital for analyzing and forecasting dynamics in time series. The integration of patching with historical data downsampling and attention mechanisms significantly improves the model's ability to accurately capture and utilize these essential temporal dependencies.

%^where $\mathbf{h}_{i,t} \in \mathbb{R}^{D}$.
%The transformer's encoder takes $\mathbf{U}_i$ as inputs, while the transformer's decoder takes $\mathbf{v}_{i,t}$ as inputs. 
%In the end, the transformer outputs $\mathbf{h}_{i,t}$ from the $N$ nodes are stacked together to from a matrix $\mathbf{H}_{:,t} = {\mathbf{h}_{1,t}, \cdots, \mathbf{h}_{N,t}\} \in \mathbb{R}^{N \times D}$. 
%This matrix $\mathbf{H}_{:,t}$ is used later to generate the time-evolving $\mathbf{M}_{t}$ and $\mathbf{A}_{t}^{adp}$, which is explained in details in \secref{sec:mainlayer}.

% We concatenate  $\{\mathbf{H}_{i}\}_{i}^{N}$ into a tensor $\mathcal{H}=\{\mathbf{H}_{:,t-T_{h}+1},\ldots, \mathbf{H}_{:,t}\} \in \mathbb{R}^{N \times T_{h}\times  D}$, where $\mathbf{H}_{:,t} \in \mathbb{R}^{N \times D}$ is the collective outputs from all node-specific transformers at timestep $t$.
% $\mathcal{H}$ is then utilized to generate the time-evolving mask matrix $\mathbf{M}_{t}$ and adjacency matrix $\mathbf{A}_{t}^{adp}$, which is further discussed in \secref{sec:mainlayer}.

% We use transformers that process the residual historical patches and standard historical observations. The patches and observations are processed first by two trainable linear layer, with the help of a learnable additive position encoding respectively:
% \begin{equation}
% \begin{gathered}
% {\mathbf{u}_{i,n}=\Hat{\mathbf{X}}_{i,n}\mathbf{W}^{u}_{i}+\mathbf{b}^{u}_{i}+\mathbf{e}_{pos}(n)}\\
% {\mathbf{v}_{i,t}={\mathbf{X}}_{i,t}\mathbf{W}^{v}_{i}+\mathbf{b}^{v}_{i}+\mathbf{e}_{pos}(t)}
% \end{gathered}
% \label{eq:fc}
% \end{equation}
% where $\mathbf{u}_{i,n} \in \mathbb{R}^D$ is the output of the $n$-th patch, $\mathbf{v}_{i,n} \in \mathbb{R}^D$ is the output of observation $\mathbf{X}_{i,t}$. $\mathbf{W}^{u}_{i} \in \mathbb{R}^{(T_{s}C)\times D}$, $\mathbf{b}^{u}_{i} \in \mathbb{R}^{D}$, $\mathbf{W}^{v}_{i} \in \mathbb{R}^{C\times D}$ and  $\mathbf{b}^{v}_{i} \in \mathbb{R}^{D}$ are learnable parameters. $\mathbf{e}_{pos}(n) \in \mathbb{R}^D$ and $\mathbf{e}_{pos}(t) \in \mathbb{R}^D$ are the position vector for $n$-th patch and observation at timestep $t$, respectively. We then collect all patch embeddings and observation embeddings into two sequences, which are denoted as $\mathbf{U}_i \in \mathbb{R}^{T_{P}\times D}$ and $\mathbf{V}_{i,t}= \{\mathbf{v}_{i,t-T_{h}+1}, \ldots, \mathbf{u}_{i,t}\}\in \mathbb{R}^{T_{h}\times D}$, respectively.
% They are finally fed into a Transformer:  
% \begin{equation}
% \mathbf{H}_{i} = {Transformer}(\mathbf{U}_i, \mathbf{V}_{i})
% \end{equation}
% where $\mathbf{H}_{i}=\{\mathbf{h}_{i,t-T_{h}+1},\ldots, \mathbf{h}_{i,t}\} \in \mathbb{R}^{T_{h}\times D}$. $\mathbf{U}_i$ and $\mathbf{V}_i$ interact through the Transformer as follows. On one hand, the transformer encoder takes $\mathbf{U}_i$ as inputs to model the temporal dependency of the residual historical data from a global view. On the other hand, the transformer decoder, it takes $\mathbf{V}_i$ as inputs. For the current timestep $t$, $\mathbf{v}_{i,t}$ can be considered as a query through the transformer decoder to extract useful information, \ie $\mathbf{h}_{i,t}$ from the residual historical data. 
% We concatenate  $\{\mathbf{H}_{i}\}_{i}^{N}$ into a Tensor $\mathcal{H}=\{\mathbf{H}_{:,t-T_{h}+1},\ldots, \mathbf{H}_{:,t}\} \in \mathbb{R}^{N \times T_{h}\times  D}$, where $\mathbf{H}_{:,t} \in \mathbb{R}^{N \times D}$ is the output representation of all nodes at timestep $t$.
% $\mathcal{H}$ is then utilized to to generate the time-evolving mask matrix $\mathbf{M}_{t}$ and adjacency matrix $\mathbf{A}_{t}^{adp}$, which is further discussed in \secref{sec:mainlayer}.


%\subsubsection{Parameterising Transformers Using Hypernetworks}

%Rather than directly learning the parameters within the aforementioned node-specific transformers, these are generated by a set of learnable hypernetworks. These hypernetworks map the node-specific spatial embedding vector, denoted as $\mathbf{e}_{i}$, to the network parameters. This, in turn, constructs the transformers for each individual node, i.e., the $i$-th node. This process is visually represented in \figref{fig:overview} with an pink background: The hypernetworks produce the weights ($W_1$,$W_2$) for multi-head attention and feed forward networks conditioned on $\mathbf{e}_{i}$, respectively.

%A significant aspect to note is that the computation involved in hypernetworks is carried out only once after the training phase. This ensures that there is no additional computational burden during the inference phase.

% Additionally, these node-specific spatial embeddings encapsulate the spatial attributes, thereby eliminating the need to model spatial dependencies between nodes. This approach completely removes the necessity for data exchange between nodes during the inference phase.

%\begin{figure}[t]
 %   \centering
  %  \includegraphics[width=0.6\linewidth]{figures/HyperTF.pdf}
   % \caption{Embedding-conditioned hypernetworks. The hypernetworks produce the weights ($W_1$,$W_2$) for multi-head attention and feed forward networks conditioned on $\mathbf{e}_{i}$, respectively.}
    %\label{fig:TF}
%\end{figure}

%We take the parameter generation process of \eqref{eq:fc} as an example to briefly introduce how hypernetworks performs:
%\begin{equation}
%\begin{gathered}
 %\medop{\mathbf{W}^{uv}_{i}=\mathbf{e}_{i}\mathbf{W}_{w}}\\
 %\medop{\mathbf{b}^{uv}_{i}=\mathbf{e}_{i}\mathbf{W}_{b}}\\
 %\medop{(\mathbf{W}^{u}_{i}, \mathbf{W}^{v}_{i}) = \operatorname{Split}(\mathbf{W}^{uv}_{i})}\\
 %\medop{(\mathbf{b}^{u}_{i}, \mathbf{b}^{v}_{i}) = \operatorname{Split}(\mathbf{b}^{uv}_{i})}
%\label{eq:hyper}
%\end{gathered}
%\end{equation}
%where $\mathbf{W}_{w} \in \mathbb{R}^{d \times(T_{s}C+1) \times D}$, $\mathbf{W}_{b} \in \mathbb{R}^{d\times 2D}$ are learnable parameters.
%$\operatorname{Split(\cdot)}$ is the operation to split a tensor into a specific number of custom-sized chunks.
%Akin to the hypernetworks described in \eqref{eq:hyper}, we can generate the weights of a transformer.
% A Transformer is stacked of Transformer layers. One transformer layer is consisted of a multi-head attention and fead-forward networks (FFN). We use hypernetworks to map the node-specific spatial embedding $\mathbf{e}_i$ to weights, which parameterise the Transformer. The details are provided in \appref{apend:tf}. 



\subsection{Dynamic Localised ASTGNNs}\label{sec:mainlayer}

Given a task time $\tau$ (as defined in Section \ref{subsec:notation}), at the timestep $t \in \{\tau-T_h+1, \cdots, \tau\}$, we need to facilitate dynamic localisation by generating of the time-evolving mask matrices $\mathbf{M}_{t}$ and adaptive adjacency matrices $\mathbf{A}_{t}^{adp}$.
% These matrices are derived from the tensor $\mathcal{H}$ provided jointly by the transformers.

% Conditioned on $\mathcal{H}$, the ASTGNNs can be dynamically localised via learning  dynamic sparse self-adaptive adjacency matrice. Given the $T_{h}$ historical observations at timestep $t$, our key approach is \textit{i)} to generate a sequence of time-vary mask matrices $\{\mathbf{M}_{t-T_{h}+1},\ldots, \mathbf{M}_{t}\}$ and \textit{ii)} to generate dynamic sparse self-adaptive adjacency matrices 
% $\{\mathbf{A}_{t-T_{h}+1}, \ldots, \mathbf{A}_{t}^{adp}\}$
% based on the mask matrices.

% \subsubsection{Dynamic Mask Generation}
% The way to get the mask matrix $\mathbf{M}_{t}$ at timestep $t$ is illustrated as follows.
% \begin{itemize}
%     \item We first apply a linear transformation to $\mathbf{H}_{:,t}\in \mathcal{H}$ to parameterize a trainable weight matrix $\mathbf{O}_{t}$:
%     \begin{equation}
%     {\mathbf{O}_{t}=(\mathbf{H}_{:,t}\mathbf{W}_{O})^{\operatorname{T}}}
%     \end{equation}
%      where $\mathbf{O}_{t} \in \mathbb{R}^{N\times N}$, $\mathbf{W}_{O}\in \mathbb{R}^{D\times N}$, $\operatorname{T}$ is the transposition operator.
%     \item  We then map the entry $o_{t}^{(i,j)} \in \mathbf{O}_{t}$ into binary "gates" using the hard concrete distribution, which is a contiguous relaxation of a discrete distribution and can approximate binary values. Accordingly, the computation of binary "gates" $o_{t}^{(i,j)}$ can be formulated as:
%     \begin{equation}
%     \begin{gathered}
%     { z \sim \mathcal{U}(0,1), s_{(i, j)}= Sig\left(\log z-\log (1-z)+\log \left(o_{t}^{(i,j)}\right)\right) / \beta}\\
%     {\bar{s}_{(i, j)}=s_{(i, j)}(\zeta-\gamma)+\gamma, m_{t}^{(i, j)}=\min \left(1, \max \left(0, \bar{s}_{(i, j)}\right)\right)}
%    \end{gathered}
%    \end{equation}
%    where $z$ is a uniform distribution, $Sig$ is a sigmoid function, $\beta$ is a temperature value and $(\zeta-\gamma)$ is the interval with $\zeta<0$ and $\gamma> 1$. 
%    Following \cite{bib:kdd23:Duan}, we set $\zeta=-0.1$ and $\gamma=1.1$ in practice. 
% \end{itemize}
% We make following notes on the generation of $\mathbf{M}_{t}$.
% \begin{itemize}
%     \item For the $i$-th node, the transposition operator $\operatorname{T}$ ensures that the corresponding $\mathbf{h}_{i,t}\in \mathbf{H}_{:,t}$ can map into the $i$-th column of $\mathbf{M}_{t}$, \ie $\mathbf{m}^{(:,i)}_{t} \in \mathbf{M}_{t}$. The $i$-th node can adaptively determine whether to receive data from which other nodes conditioned on $\mathbf{h}_{i,t}$, since $\left\|\mathbf{m}^{(:,i)}_{t}\right\|_0$ represent the in-degree of the $i$-th node.  
%     \item The mask $M_{t}$, which determines the topology of the spatial graph, depends on $\mathbf{H}_{:,t}$. Therefore, as $\mathbf{H}_{:,t}$ varies over time, the spatial graph becomes dynamic.
% \end{itemize}

\subsubsection{Dynamic Mask Generation}

The process of generating the mask matrix, $\mathbf{M}_{t}$, at timestep $t$ begins with a linear transformation applied to $\mathbf{H}_{:,t}$:
\begin{equation}
{\mathbf{O}_{t}=(\mathbf{H}_{:,t}\mathbf{W}_{O})^{\top}}
\end{equation}
where $\mathbf{W}_{O}\in \mathbb{R}^{D\times N}$ is a trainable parameter matrix. The output of this transformation, $\mathbf{O}_{t} \in \mathbb{R}^{N\times N}$, is then utilised to generate $\mathbf{M}_{t}$ through hard concrete distribution sampling. Each entry $o_{t}^{(i,j)} \in \mathbf{O}_{t}$ is converted into binary "gates" $m_{t}^{(i,j)} \in \mathbf{M}_{t}$ using the hard concrete distribution. This distribution is a continuous relaxation of a discrete distribution and can approximate binary values. The computation of the binary "gates" $m_{t}^{(i,j)}$ is expressed as follows:
\begin{equation}
\begin{aligned}
s_{t}^{(i, j)}&= sigmoid\left(\log z-\log (1-z)+\log \left(o_{t}^{(i,j)}\right)\right) / \beta\\
%\bar{s}_{t}^{(i, j)}=s_{t}^{(i, j)}(\zeta-\gamma)+\gamma,
m_{t}^{(i, j)}&=\min \left(1, \max \left(0, s_{t}^{(i, j)}(\zeta-\gamma)+\gamma\right)\right)
\end{aligned}    
\end{equation}
In this equation, $z$ is randomly sampled from a uniform distribution $z \sim \mathcal{U}(0,1)$ and $\beta$ represents the temperature value. Following \cite{bib:kdd23:Duan}, we set $\zeta=-0.1$ and $\gamma=1.1$ in practice.

For the $i$-th node, the transposition of the matrix ensures that the corresponding $\mathbf{h}_{i,t}$ can be mapped into $\mathbf{m}^{(:,i)}_{t}$, the $i$-th column of $\mathbf{M}_{t}$. This vector $\mathbf{m}^{(:,i)}_{t}$ determines whether the $i$-th node needs to receive data from other nodes, and this decision is solely dependent on $\mathbf{h}_{i,t}$. In other words, the $i$-th node can independently decide whether to receive data from other nodes without requiring any additional prior data exchange. The mask $\mathbf{M}_{t}$, which determines the topology of the spatial graph, evolves over time as it is computed from the transformer output $\mathbf{H}_{:,t}$ at time $t$.

\subsubsection{Dynamic Adaptive Graph Generation}

The NAPL-AGCN employed in ASTGNN only supports a static adjacency matrix, $\mathbf{A}^{adp}$. In order to accommodate a time-evolving $\mathbf{A}^{adp}_t$, we modify the node embedding $\mathbf{E}$ used to generate $\mathbf{A}^{adp}$ in \eqref{eq:self-adj} as follows:
\begin{equation}
\mathbf{E}_{t} =  \mathbf{E} + \mathbf{H}_{:,t}\mathbf{W}_{H}
\end{equation}
Here, $\mathbf{W}_{H} \in \mathbb{R}^{D\times d}$ are learnable parameters. The term $\mathbf{H}_{:,t} \cdot \mathbf{W}_{\mathbf{H}}$ signifies the time-evolving modification applied to the original node embedding $\mathbf{E}$. It's worth noting that even though the computation is expressed in matrix forms, each row's computation in $\mathbf{E}_t$, or $\mathbf{e}_{i,t} \in \mathbb{R}^d$, solely depends on $\mathbf{h}_{i,t}$. This implies that the computation of the node-specific time-evolving embedding, $\mathbf{e}_{i,t}$, is performed purely locally without the need for previous data exchange. This process is akin to dynamic mask generation.

To avoid calculating the entire matrix multiplication $\mathbf{E}_t \cdot \mathbf{E}_t^\top$ as in \eqref{eq:self-adj}, which would necessitate all nodes to share their own time-evolving embedding $\mathbf{e}_{i,t}$ with each other at every timestep, thereby causing substantial communication overhead, we propose using the locally available time-evolving mask vector $\mathbf{m}^{(:,i)}_{t}$. This vector already determines for the $i$-th node which neighbours it needs to communicate with at time $t$. Consequently, each element $\alpha_t^{(i, j)}$ in the time-evolving adjacency matrix $\mathbf{A}_{t}^{adp}$ is calculated in a similar fashion to the graph attention (GAT):
\begin{equation} \label{eq:adj}
\alpha_t^{(i, j)}=\left\{\begin{aligned}
\frac{\exp \left(\mathbf{e}_{i,t}{\mathbf{e}_{j,t}}^{\top}\right)}{\sum_{k \in \Psi} \exp \left(\mathbf{e}_{i,t}{\mathbf{e}_{k,t}}^{\top}\right)}\quad &, \quad m_{t}^{(i,j)} = 1 \\
0 \qquad \quad \qquad &, \quad m_{t}^{(i,j)}=0
\end{aligned}\right.
\end{equation}
Here $\Psi = \{j\ |\ m_{t}^{(i,j)} = 1\}$ is a set of the $i$-th node's neighbours in the sparse spatial graph. 
Even though the computation in \eqref{eq:adj} still necessitates the exchange of the time-evolving node embedding $\mathbf{e}_{i,t}$ among neighboring nodes, this requirement has been significantly reduced. Moreover, the node embedding $\mathbf{e}_{i,t} \in \mathbb{R}^d$ is quite small in comparison to the volume of data exchanged between adjacent nodes. Consequently, the total communication overhead necessary to support the dynamic spatial graph is minimal.

Finally, we substitute $\mathbf{A}^{adp}_t$ for $\mathbf{A}^{adp}$ in \eqref{eq:self-adj} to obtain the dynamic localised ASTGNN:
\begin{equation}
    \mathbf{Z}_{t}=\sigma\left(\mathbf{A}_{t}^{adp} \mathbf{X}_{:,t} \mathbf{E}W_{\mathcal{G}}\right)
\end{equation}

% \subsubsection{Dynamic Adaptive Graph Generation}

% The NAPL-AGCN utilized in ASTGNN supports only a static adjacency matrix, $\mathbf{A}^{adp}$. To facilitate a time-evolving $\mathbf{A}^{adp}_t$, we modify the node embedding $\mathbf{E}$ used to generate $\mathbf{A}^{adp}$ in \eqref{eq:self-adj}:
% \begin{equation}
% \mathbf{E}_{t} =  \mathbf{E} + \mathbf{H}_{:,t}\mathbf{W}_{H}\
% % \mathbf{A}^{adp}_t&={softmax}\left({ReLU}\left(\mathbf{E}_t\mathbf{E}_t^ \top \right)\right)
% \end{equation}
% Here, $\mathbf{W}_{H} \in \mathbb{R}^{D\times d}$ are learnable parameters. 
% The term $\mathbf{H}_{:,t}\mathbf{W}_{\mathbf{H}}$ represents the time-evolving modification made to the original node embedding $\mathbf{E}$.
% It is important to note that while the computation is expressed in matrix forms, the computation of each row of $\mathbf{E}_t$, or $\mathbf{e}_{i,t} \in \mathbb{R}^d$, depends solely on $\mathbf{h}_{i,t}$. In other words, the computation of the node-specific time-evolving embedding, $\mathbf{e}_{i,t}$, is carried out purely locally without the need for prior data exchange. This is similar to the process of dynamic mask generation.

% Now, we want to avoid calculating the whole matrix multiplication $\mathbf{E}_t \cdot \mathbf{E}_t^\top$ as in that in \eqref{eq:self-adj}, because this would require all nodes to exchange their own time-evolving embedding $\mathbf{e}_{i,t}$ with each other at every timestep, thus inducing a great communication overhead.
% Our solution is to use the locally available time-evoling mask vector $\mathbf{m}^{(:,i)}_{t}$, which decides already for the $i$-th node with which neighbours it needs to communicate at time $t$.
% Therefore, each element $\alpha_t^{(i, j)}$ in the time-evolving adaptive adjacency matrix $\mathbf{A}_{t}^{adp}$ is calculated as:
% \begin{equation}
% % \begin{gathered}
% \alpha_t^{(i, j)}=\left\{\begin{aligned}
% \frac{\exp \left(\mathbf{e}_{i,t}{\mathbf{e}_{j,t}}^{\top}\right)}{\sum_{k \in \Psi} \exp \left(\mathbf{e}_{i,t}{\mathbf{e}_{k,t}}^{\top}\right)}\quad &, \quad m_{t}^{(i,j)} = 1 \\
% 0 \qquad \quad \qquad &, \quad m_{t}^{(i,j)}=0
% \end{aligned}\right.
% % \end{gathered}
% \end{equation}
% Here $\Psi = \{j|m_{t}^{(i,j)} = 1\}$ is a collection of $i$-th node's neighbour in the sparse spatial graph. Finally, we substitute $\mathbf{A}^{adp}_t$ for $\mathbf{A}^{adp}$ in \eqref{eq:self-adj} and we have the dynamic localised ASTGNN:
% \begin{equation}
%     \mathbf{Z}_{t}=\sigma\left(\mathbf{A}_{t}^{adp} \mathbf{X}_{:,t} \mathbf{E}W_{\mathcal{G}}\right)
% \end{equation}

% \subsubsection{Dynamic Adaptive Graph Generation}
% NAPL-AGCN can only infer a static adjacency matrix $\mathbf{A}_{adp}$. To overcome such a problem, we introduce Dynamic Adaptive Graph Generation (DAGG), which 
% injects $\mathbf{H}_{:,t}$ into static node embeddings $\mathbf{E}$ to learn dynamic node embedding $\mathbf{E}_{t}\in \mathbb{R}^{N\times d}$.

% \begin{equation}
% \begin{gathered}
% \mathbf{E}_{t} =  \mathbf{\hat{E}}_{t}+\mathbf{E}\\
% \mathbf{\hat{E}}_{t}=\mathbf{H}_{:,t}\mathbf{W}_{\mathbf{H}}
% \end{gathered}
% \end{equation}
% Where $\mathbf{\hat{E}}_{t}\in \mathbb{R}^{N\times d}$ is the time embedding adapts to $\mathbf{H}_{:,t}$, $\mathbf{W}_{\mathbf{H}}\ in \mathbb{R}^{D\times d}$ are learnable parameters. We then can calculate the dynamic adjacency matrix $\mathbf{A}_{t}$ according to  $\mathbf{\hat{E}}_{t}$ and $\mathbf{M}_{t}$.
% We only compute $\alpha_{ij} \in \mathbf{A}_{t}$ for nodes $j\in N_{j}$, where $N_{j}$ is some neighborhood of node $i$ in the graph according to $\mathbf{M}_{t}$.
% \begin{equation}
% \begin{gathered}
% \alpha_{(i, j)}=\left\{\begin{aligned}
% \frac{\exp \left(e_{i j}\right)}{\sum_{k \in {N}_j} \exp \left(e_{i k}\right)}\qquad&for\quad m_{(i, j)} \neq 0 \\
% 0 \qquad&for \quad m_{(i, j)}=0
% \end{aligned}\right.\\
% e_{ij}=\mathbf{e}_{i,t}\mathbf{e}_{j,t}^{\operatorname{T}}
% \end{gathered}
% \end{equation}
% where $\mathbf{e}_{i,t} \in \mathbf{E}_{t}$.
% Then we use $\mathbf{A}_t$ to replace $\mathbf{A}_{adp}$ in \eqref{eq:self-adj}:
% \begin{equation}
%     \medop{\mathbf{Z}_{t}=\sigma\left(\mathbf{A}_{t} \mathbf{X}_{:,t} \mathbf{E}W_{\mathcal{G}}\right)}
% \end{equation}

% \subsubsection{Dynamic Adaptive Graph Generation}
% The NAPL-AGCN used in ASTGNN only supports a static adjacency matrix $\mathbf{A}^{adp}$. 
% To support a time-evolving $\mathbf{A}^{adp}_t$, we make a modification to the node embedding $\mathbf{E}$ used to generate $\mathbf{A}^{adp}$ in \eqref{eq:self-adj}:
% % we introduce Dynamic Adaptive Graph Generation (DAGG), which 
% % injects $\mathbf{H}_{:,t}$ into static node embeddings $\mathbf{E}$ to learn dynamic node embedding $\mathbf{E}_{t}\in \mathbb{R}^{N\times d}$.
% \begin{align}
% % \begin{gathered}
% % \mathbf{\hat{E}}_{t} &=\mathbf{H}_{:,t}\mathbf{W}_{\mathbf{H}} \\
% \mathbf{E}_{t} &=  \mathbf{E} + \mathbf{H}_{:,t}\mathbf{W}_{\mathbf{H}}\\
% \mathbf{A}^{adp}_t&={softmax}\left({ReLU}\left(\mathbf{E}_t\mathbf{E}_t^ \top \right)\right)
% % \end{gathered}
% \end{align}
% where $\mathbf{W}_{\mathbf{H}} \in \mathbb{R}^{D\times d}$ are learnable parameters.
% $\mathbf{H}_{:,t}\mathbf{W}_{\mathbf{H}}$ is the time-evolving modification made to the original node mebedding $\mathbf{E}$.
% Note that although the computation is written in matrix forms, the computation of each row of $\mathbf{E}_t$, i.e., the computation of $\mathbf{e}_{i,t} \in \mathbb{R}^d$, is only dependant on $\mathbf{h}_{i,t}$.
% In other words, the computation of node-specific time-evolving embedding $\mathbf{e}_{i,t}$ is done purely locally without the requirement of prior data-exchange, the same as in the dynamic mask generation process.
% % We then can calculate the dynamic adjacency matrix $\mathbf{A}_{t}^{adp}$ according to  $\mathbf{\hat{E}}_{t}$ and $\mathbf{M}_{t}$.
% % We only compute $\alpha_{ij} \in \mathbf{A}_{t}^{adp}$ for nodes $j\in N_{j}$, where $N_{j}$ is some neighborhood of node $i$ in the graph according to $\mathbf{M}_{t}$.
% % \begin{equation}
% % \begin{gathered}
% % \alpha_{(i, j)}=\left\{\begin{aligned}
% % \frac{\exp \left(e_{i j}\right)}{\sum_{k \in {N}_j} \exp \left(e_{i k}\right)}\qquad&for\quad m_{(i, j)} \neq 0 \\
% % 0 \qquad&for \quad m_{(i, j)}=0
% % \end{aligned}\right.\\
% % e_{ij}=\mathbf{e}_{i,t}\mathbf{e}_{j,t}^{\operatorname{T}}
% % \end{gathered}
% % \end{equation}
% % where $\mathbf{e}_{i,t} \in \mathbf{E}_{t}$.

% Finally, we use $\mathbf{A}^{adp}_t$ to replace $\mathbf{A}^{adp}$ in \eqref{eq:self-adj}:
% \begin{equation}
%     \mathbf{Z}_{t}=\sigma\left(\mathbf{A}_{t}^{adp} \mathbf{X}_{:,t} \mathbf{E}W_{\mathcal{G}}\right)
% \end{equation}

\subsubsection{Dynamic Adaptive Graph Sparsification}
Combining the time-evolving mask matrices $\mathbf{M}_{t}$ and adjacency matrices $\mathbf{A}_{t}^{adp}$, we define the procedure for dynamic adaptive graph sparsification as follows:
\begin{equation}\label{loss:3}
\mathcal{L}_{DAGS}=\sum_{t=1}^{T_a}\mathcal{L}_{t}(\theta, \mathbf{A}_{t}^{adp} \odot \mathbf{M}_t)+
\lambda \sum_{t=1}^{T_a}\left\|\mathbf{M}_{t}\right\|_0
\end{equation}
In this equation, $\mathcal{L}_{t}(\theta, \mathbf{A}_{t}^{adp}\ \odot \mathbf{M}_t)$ represents the training loss function computed with the dynamically pruned graph, which is masked by $\mathbf{M}_{t}$ at timestep $t$. $\mathcal{L}_{DAGS}$ is the objective function that can be trained end-to-end using the Adam optimiser.

% \subsubsection{Dynamic Adaptive Graph Sparsification}
% Finally, we formulate the dynamic adaptive graph sparsification proceedure as follows:
% %\begin{equation}\label{loss:1}
% %\medop{\mathcal{L}_{t}(\theta, \mathbf{A}_{t}^{adp})=\frac{\sum_{\tau \in \mathrm{T}} \sum_{v \in \mathcal{V}}\left\|\boldsymbol{y}_{t}^{(\tau, v)}-\hat{\boldsymbol{y}}_{t}^{(\tau, v)}\right\|_1}{|\mathcal{V}| \times|\mathrm{T}|}}
% %\end{equation}
% \begin{equation}\label{loss:2}
% \begin{aligned}
% \mathcal{L}_{DAGS}&=\sum_{t=1}^{T_a}\mathcal{L}_{t}(\theta, \mathbf{A}_{t}^{adp} \odot \mathbf{M}_t)+
% \lambda \sum_{t=1}^{T_a}\left\|\mathbf{M}_{t}\right\|_0,\\
% \left\|\mathbf{M}_{t}\right\|_0&=\sum_{i=1}^N \sum_{j=1}^N m_{(i, j)}, m_{(i,j)} \in \left\{0,1\right\}
% \end{aligned}
% \end{equation}
% where $\mathcal{L}_{t}(\theta, \mathbf{A}_{t}^{adp}\ odot \mathbf{M}_t)$ indicates the training loss function computed with dyanamically pruned graph, masked by $\mathbf{M}_{t}$ at timestep $t$. 
% $\mathcal{L}_{DAGS}$ is the objective function which can be trained end-to-end via Adam optimizer.

\subsection{Further Enhancements}
Here we discuss two additional enhancements made to our \sysname, which improve its efficiency further.
\subsubsection{Efficient Dynamic Localisation} 
The generation of a dynamic mask increases the time complexity to $O(T_{h} \cdot N^2)$ during inference. To address this, we significantly enhance the efficiency of \sysname by initiating from a sparse spatial graph, pre-localised using AGS. Given a pre-defined graph sparsity $p$, we first train a $p$-localised ASTGNN $\mathcal{F}(\cdot;\theta,\mathbf{A}^{a d p} \odot \mathbf{M}_{p})$ to achieve efficient inference. Here, $p$ represents the graph sparsity ($100\%$ means totally sparse), and $\mathbf{M}_{p} \in \mathbb{R}^{N \times N}$ is a mask matrix with a sparsity of $p$. Based on the $p$-localised ASTGNN, we only need to map entries $\{o_{t}^{(i,j)}|o_{t}^{(i,j)} \in \mathbf{O}_{t}, \mathbf{M}_{p}^{(i,j)}\neq 0\}$ into the corresponding $m_{t}^{(i,j)}$. This reduces the time complexity to $O((1-p) \cdot T_{h} \cdot N^2)$ during inference, which is significant considering that $p$ is normally larger than 80\%.

\subsubsection{Personalised Adaptive Graph Sparsification}
In real-world systems, the resources available to different nodes can vary. Consequently, we have implemented personalised localisation instead of global localisation. The node-independent processing of node-specific Transformer allows us to assign a unique weighting factor, $\lambda_{i}$, to adjust the degree of localisation for each node $i$:
\begin{equation}
\mathcal{L}_{PDAGS}=\sum_{t=1}^{T_a}\mathcal{L}_{t}(\theta, \mathbf{A}_{t}^{adp}, \mathbf{M}_t)+\sum_{t=1}^{T_a}\sum_{i=1}^{N}\lambda_{i}\left\|\mathbf{m}^{(:,i)}_{t}\right\|_0
\end{equation}

\begin{figure*}[ht]
    \centering
    \includegraphics[width=0.9\linewidth]{figures/PEMS_twin.pdf}
    \caption{Test accuracies of AGCRN and STG-NCDE, localised by \textit{\sysname} and AGS, evaluated on transportation datasets (PEMS03, PEMS04, PEMS07, and PEMS08). The black and yellow vertical dashed lines denote the MAE and MAPE of AGCRN and STG-NCDE when localised by AGS at a localisation degree of 80\%, respectively.}
    \label{fig:pems-mae}
\end{figure*}




% \subsection{Discussions}
% We make two notes on our \sysname.
% \subsubsection{Personalised Adaptive Graph Sparsification}
% In real-world systems, the available resources of different nodes maybe different. Therefore, it is better to perform personalised localisation rather than global localisation. Thanks to the node-independent processing of node-specific Transformer,
% we can assign node-specific weighting factor $\lambda_{i}$ to adjust the localisation-degree of each node $i$:
% \begin{equation}
% \medop{\mathcal{L}_{PDAGS}=\sum_{t=1}^{T_a}\mathcal{L}_{t}(\theta, \mathbf{A}_{t}^{adp}, \mathbf{M}_t)+\sum_{t=1}^{T_a}\sum_{i=1}^{N}\lambda_{i}\left\|\mathbf{m}^{(:,i)}_{t}\right\|_0}
% \end{equation}

% \subsubsection{Efficient Dynamic localiastion}
% Generating dynamic mask increases the time complexity of $O(T_{h}N^2)$ during inference. 
% To this end, we improve the efficiency of \sysname significantly by starting from a sparse spatial graph, pre-localised via AGS. 
% Given a pre-defined graph sparsity $p_{g}$, we first train a $p_a$-localised ASTGNN $\mathcal{F}(\cdot;\theta,\mathbf{A}_{a d p} \odot \mathbf{M}_{p_a})$ to achieve efficient inference, where $p_a$ is the graph sparsity of $\mathcal{F}(\cdot;\theta,\mathbf{A}_{a d p} \odot \mathbf{M}_{p_a})$, $p_{a}<p_{g}<1$, $\mathbf{M}_{p_a} \in \mathbb{R}^{N \times N}$ is a mask matrix with a sparsity of $p_a$.  Based on $p_a$-localised ASTGNN, we only need to map entries $\{o_{t}^{(i,j)}|o_{t}^{(i,j)} \in \mathbf{O}_{t}, \mathbf{M}_{p_a}^{(i,j)}\neq 0\}$ into corresponding $m_{t}^{(i,j)}$, which reduces the time complexity of $O(T_{h}p_{a}N^2)$ during inference.
